A Scalable Approach to Performing Multiplication and Matrix Dot-Products in Unary

Stochastic computing is a paradigm in which logical operations are performed on randomly generated bit streams. Complex arithmetic operations can be executed by simple logic circuits, resulting in a much smaller area footprint compared to conventional binary counterparts. However, the random or pseudorandom sources required for generating the bit streams are costly in terms of area and offset the advantages. Additionally, due to the inherent randomness, the computation lacks precision, limiting the applicability of this paradigm. Importantly, achieving reasonable accuracy in stochastic computing involves high latency. Recently, deterministic approaches to stochastic computing have been proposed, demonstrating that randomness is not a requirement. By structuring the computation deterministically, exact results can be obtained, and the latency greatly reduced. The bit stream generated adheres to a "unary" encoding, retaining the non-positional nature of the bits while discarding the random bit generation of traditional stochastic computing. This deterministic approach overcomes many drawbacks of stochastic computing, although the latency increases quadratically with each level of logic, becoming unmanageable beyond a few levels. In this paper, we present a method for approximating the results of the deterministic method while maintaining low latency at each level. This improvement comes at the cost of additional logic, but we demonstrate that the increase in area scales with the square root of n, where n represents the equivalent number of binary bits of precision. Our new approach is general, efficient, composable, and applicable to all arithmetic operations performed with stochastic logic. We show that this approach outperforms other stochastic designs for matrix multiplication (dot-product), which is an integral step in nearly all machine learning algorithms.

==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_PROGRAM_AUTHOR	Darren Hiebert	/dhiebert@users.sourceforge.net/
!_TAG_PROGRAM_NAME	Exuberant Ctags	//
!_TAG_PROGRAM_URL	http://ctags.sourceforge.net	/official site/
!_TAG_PROGRAM_VERSION	5.8	//
Hayes-Hybrid	ref.bib	/^@INPROCEEDINGS{Hayes-Hybrid,$/;"	P
Hayes-Hybrid	ref.bib	/^@INPROCEEDINGS{Hayes-Hybrid,$/;"	e
Hayes-Matrix	ref.bib	/^@INPROCEEDINGS{Hayes-Matrix,$/;"	P
Hayes-Matrix	ref.bib	/^@INPROCEEDINGS{Hayes-Matrix,$/;"	e
Qian08-DAC	ref.bib	/^@inproceedings{Qian08-DAC,$/;"	P
Qian08-DAC	ref.bib	/^@inproceedings{Qian08-DAC,$/;"	e
Qian11-PhD	ref.bib	/^@phdthesis{Qian11-PhD,$/;"	e
Qian11-PhD	ref.bib	/^@phdthesis{Qian11-PhD,$/;"	t
activation-btanh	ref.bib	/^@INPROCEEDINGS{activation-btanh,$/;"	P
activation-btanh	ref.bib	/^@INPROCEEDINGS{activation-btanh,$/;"	e
armin13	ref.bib	/^@article{armin13,$/;"	a
armin13	ref.bib	/^@article{armin13,$/;"	e
devon2	ref.bib	/^@INPROCEEDINGS{devon2,$/;"	P
devon2	ref.bib	/^@INPROCEEDINGS{devon2,$/;"	e
eqn:1	frontiers.tex	/^\\begin{equation} \\label{eqn:1}$/;"	l
eqn:2	frontiers.tex	/^\\begin{equation} \\label{eqn:2}$/;"	l
eqn:3	frontiers.tex	/^\\begin{equation} \\label{eqn:3}$/;"	l
eqn:4	frontiers.tex	/^\\begin{equation} \\label{eqn:4}$/;"	l
eqn:5	frontiers.tex	/^\\begin{equation} \\label{eqn:5}$/;"	l
eqn:6	frontiers.tex	/^\\begin{equation} \\label{eqn:6}$/;"	l
eqn:7	frontiers.tex	/^\\begin{equation} \\label{eqn:7}$/;"	l
fig:1	frontiers_SupplementaryMaterial.tex	/^\\caption{ Enter the caption for your figure here.  Repeat as  necessary for each of your figures}\\label{fig:1}$/;"	l
fig:2	frontiers_SupplementaryMaterial.tex	/^\\caption{This is a figure with sub figures, \\textbf{(A)} is one logo, \\textbf{(B)} is a different logo.}\\label{fig:2}$/;"	l
fig:AccuracyComparison	frontiers.tex	/^\\label{fig:AccuracyComparison}$/;"	l
fig:ClkDiv	frontiers.tex	/^\\label{fig:ClkDiv}$/;"	l
fig:ClkDiv2	frontiers.tex	/^\\label{fig:ClkDiv2}$/;"	l
fig:Conv	frontiers.tex	/^\\label{fig:Conv}$/;"	l
fig:Conventional_Drawback	frontiers.tex	/^\\label{fig:Conventional_Drawback}$/;"	l
fig:GateCost1	frontiers.tex	/^\\label{fig:GateCost1}$/;"	l
fig:GateCost2	frontiers.tex	/^\\label{fig:GateCost2}$/;"	l
fig:MultiAdd	frontiers.tex	/^\\label{fig:MultiAdd}$/;"	l
fig:Stochastic-Neuron	frontiers.tex	/^\\label{fig:Stochastic-Neuron}$/;"	l
fig:Stochastic_Representation	frontiers.tex	/^\\label{fig:Stochastic_Representation}$/;"	l
fig:Thermometer_Encoding	frontiers.tex	/^\\label{fig:Thermometer_Encoding}$/;"	l
fig:case3a	frontiers.tex	/^\\label{fig:case3a}$/;"	l
fig:case3b	frontiers.tex	/^\\label{fig:case3b}$/;"	l
fig:case3c	frontiers.tex	/^\\label{fig:case3c}$/;"	l
fig:clock_div_circuit	frontiers.tex	/^\\label{fig:clock_div_circuit}$/;"	l
fig:clock_div_example	frontiers.tex	/^\\label{fig:clock_div_example}$/;"	l
fig:downscale_1	frontiers.tex	/^\\label{fig:downscale_1}$/;"	l
fig:downscale_2	frontiers.tex	/^\\label{fig:downscale_2}$/;"	l
fig:final_circuit_a	frontiers.tex	/^\\label{fig:final_circuit_a}$/;"	l
fig:final_circuit_b	frontiers.tex	/^\\label{fig:final_circuit_b}$/;"	l
fig:unary_generator	frontiers.tex	/^\\label{fig:unary_generator}$/;"	l
fixed-length	ref.bib	/^@article{fixed-length,$/;"	a
fixed-length	ref.bib	/^@article{fixed-length,$/;"	e
gaines	ref.bib	/^@inproceedings{gaines,$/;"	P
gaines	ref.bib	/^@inproceedings{gaines,$/;"	e
lfsrs	ref.bib	/^@INPROCEEDINGS{lfsrs,$/;"	P
lfsrs	ref.bib	/^@INPROCEEDINGS{lfsrs,$/;"	e
li2012	ref.bib	/^@INPROCEEDINGS{li2012,$/;"	P
li2012	ref.bib	/^@INPROCEEDINGS{li2012,$/;"	e
parhi1	ref.bib	/^@ARTICLE{parhi1,$/;"	a
parhi1	ref.bib	/^@ARTICLE{parhi1,$/;"	e
parhi2	ref.bib	/^@inproceedings{parhi2,$/;"	P
parhi2	ref.bib	/^@inproceedings{parhi2,$/;"	e
qian2008	ref.bib	/^@INPROCEEDINGS{qian2008,$/;"	P
qian2008	ref.bib	/^@INPROCEEDINGS{qian2008,$/;"	e
qian2011	ref.bib	/^@ARTICLE{qian2011,$/;"	a
qian2011	ref.bib	/^@ARTICLE{qian2011,$/;"	e
riedel1	ref.bib	/^@article{riedel1,$/;"	a
riedel1	ref.bib	/^@article{riedel1,$/;"	e
riedel2	ref.bib	/^@article{riedel2,$/;"	a
riedel2	ref.bib	/^@article{riedel2,$/;"	e
riedel3	ref.bib	/^@article{riedel3,$/;"	a
riedel3	ref.bib	/^@article{riedel3,$/;"	e
sec:HardwareImplementation	frontiers.tex	/^\\section {Hardware Implementation}\\label{sec:HardwareImplementation}$/;"	l
sec:OurApproach	frontiers.tex	/^\\section {Scalable Deterministic Approach} \\label{sec:OurApproach}$/;"	l
sec:Proof	frontiers.tex	/^\\section {Mathematical Proof}\\label{sec:Proof}$/;"	l
sec:Results	frontiers.tex	/^\\section {Simulation and Results} \\label{sec:Results} $/;"	l
sec:background	frontiers.tex	/^\\section{Background Information} \\label{sec:background}$/;"	l
sec:conclusion	frontiers.tex	/^\\section {Conclusion} \\label{sec:conclusion}$/;"	l
sobol	ref.bib	/^@INPROCEEDINGS{sobol,$/;"	P
sobol	ref.bib	/^@INPROCEEDINGS{sobol,$/;"	e
sobolckt	ref.bib	/^@article{sobolckt,$/;"	a
sobolckt	ref.bib	/^@article{sobolckt,$/;"	e
ssec:Arithemetic_Functions_Results	frontiers.tex	/^\\subsection{Arithmetic Functions} \\label{ssec:Arithemetic_Functions_Results}$/;"	l
ssec:DoubleMultiplication	frontiers.tex	/^\\subsection {Multiplication within an Operation} \\label{ssec:DoubleMultiplication}$/;"	l
ssec:Matrix_Multiplication	frontiers.tex	/^\\subsection{Matrix Multiplication} \\label{ssec:Matrix_Multiplication}$/;"	l
ssec:Multiplication_Results	frontiers.tex	/^\\subsection{Multiplication} \\label{ssec:Multiplication_Results}$/;"	l
ssec:background_1	frontiers.tex	/^\\subsection{Introduction to Stochastic Computation} \\label{ssec:background_1}$/;"	l
ssec:deterministic_downscaling_2	frontiers.tex	/^\\subsection {Downscaling} \\label{ssec:deterministic_downscaling_2}$/;"	l
ssec:error_compensation	frontiers.tex	/^\\subsection{Error Compensation} \\label{ssec:error_compensation}$/;"	l
ssec:recap	frontiers.tex	/^\\subsection{The Deterministic Approach to Stochastic Computing} \\label{ssec:recap}$/;"	l
survey	ref.bib	/^@article{survey,$/;"	a
survey	ref.bib	/^@article{survey,$/;"	e
tab:AccuracyComparison	frontiers.tex	/^\\label{tab:AccuracyComparison}$/;"	l
tab:AccuracyComparison2	frontiers.tex	/^\\label{tab:AccuracyComparison2}$/;"	l
tab:Lenet-test	frontiers.tex	/^\\label{tab:Lenet-test}$/;"	l
tab:Matrix-MAE	frontiers.tex	/^\\label{tab:Matrix-MAE}$/;"	l
tab:Progressive Accuracy	frontiers.tex	/^\\label{tab:Progressive Accuracy}$/;"	l

